On-edge Multi-task Transfer Learning: Model and Practice with Data-driven Task Allocation

On edge devices, data scarcity occurs as a common problem where transfer learning serves as a widely-suggested remedy. Nevertheless, transfer learning imposes a heavy computation burden to resource-constrained edge devices. Existing task allocation works usually assume all submitted tasks are equally important, leading to inefficient resource allocation at a task level when directly applied in Multi-task Transfer Learning (MTL). To address these issues, we first reveal that it is crucial to measure the impact of tasks on overall decision performance improvement and quantify \emph{task importance}. We then show that task allocation with task importance for MTL (TATIM) is a variant of the NP-complete Knapsack problem, where the complicated computation to solve this problem needs to be conducted repeatedly under varying contexts. To solve TATIM with high computational efficiency, we propose a Data-driven Cooperative Task Allocation (DCTA) approach. Finally, we evaluate the performance of DCTA by not only a trace-driven simulation, but also a new comprehensive real-world AIOps case study that bridges model and practice via a new architecture and main components design within the AIOps system. Extensive experiments show that our DCTA reduces 3.24 times of processing time, and saves 48.4\% energy consumption compared with the state-of-the-art when solving TATIM.

==> CRL-model.tex <==
\section{Clustered Reinforcement Learning (CRL) Model}\label{Sec:Model}
In this section, we first present an overview of the data-driven approach for task allocation. We then introduce the background of reinforcement learning. At last, we give a formal definition of the environment-dynamic task allocation and propose our data-driven approach using Clustered Reinforcement Learning (CRL).

\subsection{Data-driven Task Allocation Overview}
In the previous section, we show that our TATIM problem is in general 1) NP-complete 2) with time-varying parameters, leading to complicated computations conducted repeatedly. The key to efficiently allocate tasks on the edge lies in the automatically adaptation to varying contexts.

As a remedy to such a challenge, we then propose the data-driven task allocation. Recent years have witnessed a trend of applying data-driven techniques for complicated problems in time-varying environments, including AlphaGO \cite{silver2016mastering}, Intelligent logistics \cite{li2018development}, Autonomous Mobility-on-Demand system \cite{iglesias2018data} and Human-level game control \cite{mnih2015human}. Basically, data-driven techniques are particularly helpful for solving complicated problems repeatedly with varying parameters, because they not only help to model and reduce the environmental randomness in multi-task scenarios but also help to significantly enhance the computational efficiency due to the fast inference phase when the solution is needed.\footnote{Though the training phase may be long, it merely needs to be conducted once in advance.} 


Formally, given a task set $\textbf{J}$ and the corresponding historical feature space $\mathcal{X}$, we are to develop a data-driven task allocation scheme with a loss function $\mathcal{L(\cdot)}$ which maximize the overall decision performance of the task allocation, i.e.,
\begin{equation*}
\begin{aligned}
\textbf{u} \leftarrow \mathcal{F(\textbf{J},\mathcal{X})}.
\end{aligned}
\end{equation*} 
 
 %Accordingly, in the rest of this section, we model our optimization as a Markov decision process and propose our data-driven approach using Clustered Reinforcement Learning (CRL). Due to the simulation limitation of CRL, we further propose a Cooperative Learning approach based on both CRL and Support Vector Machine (SVM) to fully leverage the simulated and real-world data. A framework and case study is also available in Section \ref{Sec:CaseStudy} showing how we leverage the task allocation and the benefit in a practical scenario.

\subsection{Background of Reinforcement Learning}

Next, we consider the proper approach to solve the TATIM problem. 
First, in the previous section, we have proved that the TATIM problem is in fact a Knapsack problem and therefore NP-complete. Reinforcement learning (RL) is widely suggested to efficiently solve such problems \cite{mnih2015human,silver2016mastering}. 
Second, decisions made by industrial systems can be highly repetitive, thus generating an abundance of training data to support complicated data-driven model. 
Based on the two reasons, we applied the well-known RL to solve the TATIM problem.  

In general, the RL works like this: at each decision epoch, the agent will make a decision based on the current state of the environment. Once the decision is made, a reward would be provided to the agent and the state of the environment would be updated for making future decisions. The agent tries to maximize the cumulative rewards over time.
With RL, our TATIM problem is optimized in a Markov Decision Process (MDP), which is a five-tuple: $<\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \lambda>$,  where $\mathcal{S}$ denotes the set of states; $\mathcal{A}$ denotes the set of actions; $\mathcal{P}$ denotes the transition probability distribution; $r$ denotes the reward function and $\lambda \in [0,1]$ denotes the discount factor for future rewards. Note that different optimization problems have quite different objectives, constraints, and variables. To adopt our TATIM problem, the different components of RL needs to be specially designed. The detailed design of these components in RL and MDP will be discussed next.


\subsection{Environment-dynamic Task Allocation} 
However, RL should not be directly applied in our scenario, where the environment is diverse over time and existing RL approaches usually assume a fixed environment.

\textbf{Novel Problem of Environment-dynamic Knapsacks.} In TATIM, the task importance is critical for environment modeling and thus also important for RL. As we known, the knowledge learned by the decision of an agent is rewarded according to the environment. Once the task importance and the corresponding environment is not close to reality, the decision made by the agent will lead to poor decision performance. 

However, due to the varying scenarios in MTL, the environment matrix of RL usually changes over time in reality. Recall the previous example where a self-driving car on the highway and pedestrians usually do not occur, the task of pedestrians detection is less important compared to other tasks. Nevertheless, when driving around the school, pedestrians are particularly frequent which makes the task of pedestrians detection more important. Therefore, we see that the environment is clearly diverse in different scenarios, especially when the task importance is encoded in the environment of RL.\footnote{Even in the same scenario, the environment can change over time, due to the accumulating size of training data and the overwritten historical data when the storage is insufficient. An experiment in the previous section also indicates the fluctuation between historical and current task importance.}
 
In this regard, directly leveraging the RL model can easily mismatch the environment and submitted less important tasks, which leads to poor decision performance \cite{bai2015information,hu2018synthesize}. We also conduct an experiment to demonstrate the negative impact. It shows a 46.28\% reduction of performance when the environment is not accurate using existing RL. 

To this end, we realize that our TATIM problem can be regarded as a novel variant of the Knapsack problem. It is even more challenging than the Multiply-constrained Multiple Knapsack Problem proved in the previous section. This time, additionally, the item value (i.e., task importance) can be changed randomly over time, instead of being fixed in the traditional Knapsack problem. 

\textbf{Clustered Approach for Environment Definition.} Accordingly, to solve the TATIM problem, we are to learn the current environment. Our idea is that the more similar historical days, the more similar the environment is. Such similarity can be measured by comparing the current scenarios and configuration settings, e.g., sensing data, of the predicting day and the historical days. 

The overall process is illustrated in Fig.~\ref{fig:dynamic-environment}, which consists of two parts, i.e., environment definition and data-driven task allocation. In the figure, different days represent different environments, and the darkness of each color represents the different task importance. Through the analysis of historical data, we establish an environment data set, i.e., historical environment $\mathcal{E}$. We define the historical environment $\mathcal{E}$ as the collection of environment $e$, i.e.,
\begin{eqnarray*}
\mathcal{E} = [e_{1}, e_j,\cdots,e_{N'}],\ \ \  \forall j \in [1,2,\cdots,N'],
\end{eqnarray*}
where $e_j$ denotes the corresponding environment. For better understanding, a formal mathematical structure of the environment is available in the following Section III-D. 

Through environment definition that we can find a similar environment $e$ by clustering algorithms such as \emph{k Nearest Neighbors} (kNN), i.e.,
\begin{eqnarray*}
e = kNN(\mathcal{E},Z), 
\end{eqnarray*}
where $Z$ denotes the sensing data. We then can make data-driven task allocation based on the clustered environment under the execution time and resource constraints. 


\begin{figure}[t]
\centering
\vspace{-0.1cm}
\includegraphics[angle=0, width=0.45\textwidth]{figures/Environment-dynamic_task_allocation.pdf}
\vspace{-0.2cm}
\caption{The illustration of environment-dynamic task allocation.} 
\label{fig:dynamic-environment}
\vspace{-0.5cm}
\end{figure}


\subsection{Clustered Reinforcement Learning for Environment-dynamic Task Allocation} 
Next, we propose key designs of our approach, i.e., the environment modeling, state space, action space, reward function, and optimization, which should be specified based on our TATIM problem.

\textbf{Environment.} A key component in the RL model is the \emph{environment}, which is everything outside the agent, and changes its state due to the action of the agent, and gives the agent corresponding rewards. For an RL predictor, the environment can be described as a matrix $e$ which is a map of the agent, e.g., Maze problem. More specifically, one dimension represents the subject types (e.g., neighboring car detection, traffic sign detection, and pedestrian detection), and the other represents the available processors (CPU processor, GPU processor, sensors). The elements of the matrix can be viewed as a data-driven task. It is formulated as follows:
\begin{eqnarray*}
e = [I_{j}\times V_p]_{N \times M},\ \ \  \forall I_{j}, V_p \in \mathbb{R},
\end{eqnarray*}
where $I_{j}$ denotes the corresponding task importance and $V_p$ denotes the corresponding processor capacity.

\textbf{State space.} We represent the state, which is the current task selection of the system. More specifically, the state is defined by a matrix $\mathcal{S}$ and the element of each position can be 0 or 1. Note that 1 represents the task is selected, otherwise, it is not selected, which is formulated as follows: 
\begin{eqnarray*}
\mathcal{S} = [s_{ij}]_{N \times M},\ \ \  \forall s_{ij} \in \{0,1\}
\end{eqnarray*}
Such a fixed state representation indicates that it can be conveniently applied as an input to a neural network.

\textbf{Action space.} At each point in time, the scheduler may want to select any subset of the $N\times{M}$ tasks. But this requires a large action space of size $2^{N\times{M}}$ leading to unbearable computation to learn on the edge. We keep the action space small using a trick: we allow the agent to execute merely one action in each time step. The action space is given by $\{{1,2,\cdots,M}\}$, where $a$ = ${j}$ means to conduct the $j^{th}$ task for the current processor in the current time step. Hence, the action space is defined as follows:
\begin{eqnarray*}
\mathcal{A} = \{ a|a \in \{ 1,2,\cdots,M \} \} 
\end{eqnarray*}
In this way, we can greatly speed up our learning rate while keeping the action space linear in $M$.


\textbf{Reward Function.} We craft the reward signal to guide the agent towards desired solutions for our objective: maximize overall task importance. Specifically, we set the reward at each time step to $\sum_{j \in \textbf{J}} I_j$ only if the agent reaches the terminal state (i.e., all tasks in the current system are assigned accordingly), where $\textbf{J}$ is the set of tasks currently in the system. Otherwise, the reward was set to 0. Hence, 
\begin{eqnarray*}
r(t) = 
\begin{cases} 
\sum_{j \in \textbf{J}} I_j, & \mbox{if the agent reaches the terminal state } 
\\ 0, & \mbox{otherwise.}
\end{cases} 
\end{eqnarray*}

It is worth noting that the agent is set to not receive any reward for intermediate decisions during a time step, which is well-suited to apply to our real-world decision objectives.



\begin{algorithm}[t]
\caption{Clustered Reinforcement Learning (CRL)}\label{alg:CRL}
\begin{algorithmic}[1]
\Require
\State $\bm{\mathcal{E}} \gets$ historical environment \ \ $s_0 \gets$ initial state \ \ $Z \gets$ current scenarios and configuration settings.
\State $e \gets$ \emph{EnvironmentDefinition}($\bm{\mathcal{E}}$,$Z$) \Comment{Find similar environment.} 
\While{not yet reach the terminal state $s_N$}	 \label{alg:sc}
  \State $\mathcal{L}(s,a| \theta) \gets (r + \max \limits_{a} Q(s',a| \theta) - Q(s,a| \theta))^2$  \Comment{Update DNN parameters $\theta$.}
\EndWhile 
  \State $\bm{\theta ^*} \gets \arg \min \mathcal{L}(s,a| \theta)$  \Comment{Obtain optimal parameter $\theta$.}
 \State \Return $e, \ s_0,\ \bm{\theta ^*}$
\Ensure
\State $(e, \ s_0,\  \bm{\theta ^*})$ $\leftarrow$ initialization using the return value of the training phase.
\State $\textbf{u} \leftarrow \mathcal{F}_1((e,s_0);\bm{\theta ^*})$ \Comment{Make task allocation prediction.}
\State \Return $\textbf{u}$
\end{algorithmic}
\end{algorithm}


\textbf{Optimization.} With the above key elements, we leverage Deep Q-learning $Q(s,a; \theta, \textbf{J})$ \cite{liu2017hierarchical}, where $\theta$ denotes the adjustable parameter vector of neural networks. It estimates the value of executing an action $a$ from a given state $s$. Formally, given the feature space $\mathcal{X}$ which consist of the environment $e$ and the initial state $s_0$, we have
\begin{eqnarray}
\textbf{u} \leftarrow \mathcal{F}_1(\textbf{J},\mathcal{X}) = \mathcal{F}_1(\textbf{J},(e,s_0)) = Q(s,a;\theta,\textbf{J}).
\end{eqnarray}

Based on the above design, we propose the Clustered Reinforcement Learning (CRL) approach, as shown in Algorithm~\ref{alg:CRL}.


\textbf{Convergence Analysis.} It has been proven that the Deep Q-learning technique will gradually converge to the optimal policy under stationary Markov decision process (MDP) environment and sufficiently small learning rate \cite{watkins1992q}. Hence, the proposed CRL predictor will converge to the optimal policy when (i) the environment evolves as a stationary, memoryless Semi-Markov Decision Process and (ii) the DNN is sufficiently accurate to return the action associated with the optimal $Q(s, a)$ estimate.






==> CaseStudy-back.tex <==
\section{Case Study: Chiller AIOps on the Edge}\label{Sec:CaseStudy}

{An important application of multi-task transfer learning on the edge is \emph{AIOps}. The term \emph{AIOps}~\cite{lerner18} is coined as a system that utilizes big data, machine learning and other advanced analytics to enhance IT operations, such as monitoring, automation, and service desk, with proactive, customized and dynamic insight. Data-driven analytics have been widely suggested for IT Operations Management. According to Gartner Inc., by 2022, 40\% of all large enterprises will adopt AIOps systems \cite{cappelli18}.}

{The industry AIOps system usually consists of two stages, i.e., Data-driven Multi-task Transfer Learning and Final Optimization, and they work as follows. First, when an industrial demand arrives, AIOps systems need to choose a series of data-driven prediction tasks to conduct, e.g., by using Data-driven Multi-task Transfer Learning. Second, it comes to Final Optimization. In this stage, the AIOps systems receive all the results of previous prediction tasks and conduct decisions until the decision performance, i.e., overall merit, is no longer improved.} 

%\todo{It may not be necessary to conduct in a iterative manner for all tasks so that I remove the previous description.}

%In this section, we focus on applying our data-driven cooperative task allocation (DCTA) approach to the real-world edge-computing system. We first present the overview of AIOps system. We then briefly introduce the system framework and main components design within our system. Finally, through real experiments demonstrate the superiority of our system.


{In this section, we focus on applying our data-driven cooperative task allocation (DCTA) approach to the real-world edge-computing system. We first introduce the background of Industry AIOps and observe the operation redundancy exist. We then present the overview of AIOps system and briefly introduce the system architecture and main components design within our system. Finally, through real experiments demonstrate the superiority of our system.}


\begin{figure}[t]
\centering
\vspace{-0.1cm}
\includegraphics[angle=0, width=0.3\textwidth]{figures/operation.pdf}
\vspace{-0.3cm}
\caption{The probability of becoming the best operation for different machines.}
\label{fig:operation}
\vspace{-0.3cm}
\end{figure}



\subsection{Overview of DCTA in Chiller AIOps System}
{As a case study, the \emph{chiller AIOps system}, i.e., AIOps system conducting chiller operations, is deployed for one week on January, 2019, in a high-rise office building which serves more than three thousand people. Chiller is a machine generate cooling power in commercial buildings and chiller operation is a significantly important operation, which aims to select run-time configurations of the chiller so that the overall system serves the cooling demand while minimizes the electricity consumption. For example, conducting chiller operations in a building with two chillers [0.5, 0.7] implies that chiller 1 and chiller 2 are operating at 50\% and 70\% of their maximum rated capacity, respectively. Chiller AIOps system has been studied recently to significantly improve energy efficiency in commercial buildings and this case study is conducted based on a real-world chiller operation dataset~\cite{zheng2018data}. Here, the efficacy of chiller operation control relies heavily on the {\it run-time} performance profile of the chillers, namely the COP under different cooling load regimes. COP is a measure of the energy-efficiency of a chiller and captures the cooling power that it can output for a certain input power consumption \cite{wiki19}. Formally,
\begin{eqnarray*}
\emph{COP}_i =  Q_{i} / E_{i},
\end{eqnarray*}
where $E_i$ is the electrical power consumed by chiller $i$ to deliver the required amount of cooling load $Q_i$.}

%\todo{Try not to cite our paper here: please use the origin reference in our e-energy paper} \todo{Please add more COP prediction paper}

{Reliable chiller operations depend on the COP across all the loading conditions for chiller $i$. However, besides the well-known fact that COP degrades over time~\cite{yu08,firdaus16}, COP also fluctuates markedly over different cooling loads and environmental conditions~\cite{zheng2018data}, which makes it exceedingly difficult to capture within an analytical model. To this end, data-driven techniques can thus play a crucial role in accurate COP prediction for improved chiller operations in chiller AIOps system. Specifically, a \emph{learning task} is defined as the coefficient of performance (COP) prediction of a chiller for one particular operation and works have been proposed for chiller AIOps~\cite{michopoulos07,powell13,hartman14,zheng2018data}. After COPs of operations is predicted, chiller operations conducted by selecting operation with the highest COP value to meet the cooling demand with the lowest electricity consumption.}



\begin{figure}[t]
\centering
\vspace{-0.1cm}
\includegraphics[angle=0, width=0.48\textwidth]{figures/hvacReal.pdf}
\vspace{-0.2cm}
\caption{Chiller AIOps System on the Edge.}
\label{fig:hvacReal} 
\vspace{-0.3cm}
\end{figure} 



\begin{figure*}[t]
	\begin{minipage}[htpb]{0.48\linewidth}
		\centering
		%\vspace{-0.1cm}
		\includegraphics[width=2.75in]{new-figure/topology.pdf}
		%\vspace{-0.2cm}
		\caption{The Network Topology of Chiller AIOps System on the Edge. \label{fig:topology}}
	\end{minipage}
	\hfill
	\begin{minipage}[htpb]{0.48\linewidth}
		\centering
		%\vspace{-0.2cm}
		\includegraphics[width=3.5in]{new-figure/framework.pdf}
		\vspace{-0.5cm}
		\caption{Architecture Overview of Chiller AIOps System on the Edge. \label{fig:framework}}
	\end{minipage}
	\hfill
\vspace{-0.3cm}
\end{figure*}

%\todo{We need to carefully define task here. Reader will not understand COP prediction. We may either 1. Explain the concept of COP and its relation to chiller operation (in fact, operation conducted by selecting operation with the highest COP value, by meeting the cooling demand); or 2. directly says we are predicting the chiller performance, which is predicting the energy cost of different operations.} 

{\textbf{Motivation of DCTA in Chiller AIOps.} The chiller operation process requires performance predicted across all possible operations. There are too many controllable parameters in the industry and the number of parameter combinations is usually huge for all possible operations. However, the chiller operation process is typically accompanied by time limits, e.g., two hours for chiller operations \cite{sun13}. A previous study indicates that blindly conducting all learning tasks leads to considerable time consumption which easily exceeds the time limits in chiller operation~\cite{zheng2018data}. When merely partial operations are conducted in random order and these operations fail to meet the cooling demand, the backup chiller plant would be launched and additionally consumes a large amount of electricity. Therefore, we can conduct the proposed task allocation which assigns more important tasks to more powerful edge devices for priority execution under time limits.}



{Based on the above real-world industrial dataset, while in principle all COP entries (i.e., learning tasks) may be selected to conduct the chiller operations, in practice only a small subset of them are frequently selected in the optimal operation. The historical best operations can be computed with the final optimization based on the ground truth of COP of 1460 days from 2012 to 2015. Then we can count the number of cases for each operation to be selected as the best operation and thus obtain the probability to become optimal. For example, if an operation is selected in 100 days as the best operation over the total 1460 days, its probability to become optimal is computed as 100 / 1460 = 6.84\%. Fig.~\ref{fig:operation} shows that the probability of becoming the best operation for different machines vary greatly among the exponential optional operation space. It can be seen that there merely a small portion of operations are frequently selected. Results also confirm our previous Observation 1 in Section~\ref{Sec:observation}.}

%{Based on the above real-world industrial dataset, we make an observation that is shown in Fig. \ref{fig:operation}, where the probability of becoming best operation for different machines vary greatly among the exponential optional operation space. It can be seen that there merely a small portion of operations are frequently selected. Results also confirm our previous Observation 1 in Section~\ref{Sec:observation}.} \todo{Please describe the figure first, before dumping to observation results.}





{\textbf{Task Importance in Chiller AIOps.} The key of the DCTA lies in the computation of task importance. Next, in the context of this AIOps case study, we formally present a specified formulation of the \emph{task importance} computation.} 

As discussed in previous Definition 1 in Section~\ref{Sec:notation}, given model parameters $\bm\theta$, the task importance $\mathcal{I}_j$ can be updated using the merit function $\mathcal{H}(\cdot)$. For interested readers, a more concrete definition of $\mathcal{H}(\cdot)$ is also available in Section~\ref{Sec:notation}, where involved two following important concepts, i.e., the ideal electricity consumption $D$ and decision-making function $\mathcal{D}(\cdot)$. Specifically, as for $D$, we first find the best operation (i.e., with the highest COP value) in each day through the historical ground truth of COP data, and then compute the electricity consumption of conducting this operation as the ideal performance.

{Next, the decision-making function $\mathcal{D}(\cdot)$ is intrinsically solving an optimization problem finding the best chiller operations which minimize the total electricity consumption on one day where all time instances in one day are denoted by $T$ and each operation is conducted at time $t \in T$. Let $L_i$ denote the maximum cooling capacity of chiller $i < n$ and $S_{i, t}$ denote the partial load ratio of chiller $i$ at time $t$. Formally,
\begin{equation*}\label{Eq:decision}
    \begin{aligned}
    \mathcal{D}(\bm{\theta}) = \min  \limits_{\bm\theta} 
    \sum_{t=1}^{T} \sum^n_{i=1} L_i \cdot S_{i, t} / COP_{i, t}\\ 
    \mbox{ s.t.}
    \sum^n_{i=1} Q_i > \mathcal{D}\ \ and\ \ T_N \leq T_D,
    \end{aligned}
\end{equation*}
where $COP_{i, t}$ denotes the data-driven prediction performance of chiller $i$ at time $t$; $Q_i$ and $\mathcal{D}$ respectively denote the cooling load produced by chiller $i$ and the total cooling demand; $T_N$ and $T_D$ denote the total processing time and the deadline, respectively. More specifically, the deadline $T_D$ here means the total time length of one chiller operation, including the computation time and the mechanical switching time, computed considering both the periodic interval $t_P$ and mechanical switching time $t_M$, e.g., $T_D = \min(t_P, t_M)$ \cite{zheng2018data}.}


% {As discussed in previous Definition 1 in Section~\ref{Sec:observation}, given model parameters $\bm\theta$, the task importance $\mathcal{I}_j$ can be updated using the merit function $\mathcal{H}(\cdot)$. Formally,
% \begin{eqnarray*}
% \mathcal{H}(\bm{J};\bm\theta) = 1- \frac{|D - \mathcal{D}(\bm{J};\bm{\theta})|}{D},
% \end{eqnarray*}
% where $\mathcal{D}(\cdot)$ is the decision-making function given model parameters and $D$ denotes the ideal electricity consumption which can be computed through the historical data. Specifically, as for $D$, we first find the best operation in each day through the historical data and compute the electricity consumption of conducting this operation as the ideal performance.}

%\todo{Since overall merit has been defined, redefine merit function seems to be redundant. My suggestion is: 1. As for H(), Here we merely need brief introduce and reference to previous section. 2. We can talk about the computation of D (how do we get the ideal electricity consumption).}

%\todo{I move the specific computation for D here. But talking about finding the best performance, we mentioned that we need to find the best operation each day. So a natural question would be: how do we know the best operation then?}


%\todo{As another key difference against the conference version, we can formally/ mathmatically specify what are the $\mathcal{H}(\cdot)$ function and the $\mathcal{D}(\cdot)$ function used in Chiller AIOps in details.}




\subsection{Device Overview} \label{sec:casestudy}
{According to above, we conduct the task allocation based on the chiller AIOps system in the Pacific Place, Hong Kong, where the network topology is shown in Fig.~\ref{fig:topology}. The equipment of chillers, pumps, air-handling unit, and cooling tower differ greatly in operation, maintenance, and services. The data of each equipment in the chiller plant (Fig.~\ref{fig:hvacReal}~A.1) are captured and transmitted by 13 edge nodes, including 3 operation nodes (from the vendor of Trane, Fig.~\ref{fig:hvacReal}~A.2) conducting and recording operations, and 10 sensing nodes (from the vendor of Schneider Electric, Fig.~\ref{fig:hvacReal}~A.2) collecting sensing data. To process data from different types of equipment, we choose a centralized approach, where edge node transmits data to the controller (from the vendor of Wago, Fig.~\ref{fig:hvacReal}~A.3), and controllers are responsible for task allocation and decision making for the edge nodes. Finally, 3 operation nodes conduct data-driven COP prediction and send control sequences to devices (Fig.~\ref{fig:hvacReal}~B). Other sensing nodes without computation power are merely used to collect data.}

{Though hardware can be fully redeployed after introducing data-driven techniques~\cite{agyapong14}, for the scalability purpose, we choose an incremental deployment for the chiller AIOps system, with minimal revision for the current HVAC system. That is to say, we leverage only the current commercial off-the-shelf components and avoid deploying any additional equipment within the HVAC system. However, we may sacrifice the probability to obtain more sensing data and have even better prediction performance, if we avoid deploying additional equipment inside the local system in each building for the scalability purpose.}

\begin{figure*}[ht]
    \vspace{-0.1cm}
	\begin{minipage}[htpb]{0.32\linewidth}
		\centering
		\vspace{-0.18cm}
		\includegraphics[width=2.45in]{figures/overallmerit.pdf}
		\vspace{-0.8cm}
		\caption{The overall merit as a function of the number of performed tasks. \label{fig:merit}}
	\end{minipage}
	\hfill
	\begin{minipage}[htpb]{0.32\linewidth}
		\centering
		\vspace{-0.2cm}
		\includegraphics[width=2.4in]{figures/processtime.pdf}
		\vspace{-0.74cm}
		\caption{The processing time of task allocation system with different number of tasks. \label{fig:time}}
	\end{minipage}
	\hfill
	\begin{minipage}[htpb]{0.32\linewidth}
		\centering
		\vspace{0.2cm}
		\includegraphics[width=2.4in]{figures/energyconsumption.pdf}
		\vspace{-0.8cm}
		\caption{The energy consumption of task allocation system with different number of tasks. \label{fig:energy}}
	\end{minipage}
	\hfill
\vspace{-0.5cm}
\end{figure*}

\subsection{Component Designs} 
{To apply our Data-driven Cooperative Task Allocation (DCTA)  approach to the chiller AIOps system, we also introduce the architecture overview of our chiller AIOps system, as shown in Fig. \ref{fig:framework}. The architecture contains four main modules: (1) {\em Data Collecting Module} collects the data from the surroundings for analysis. Not only the current data but also the historical data are needed to be collected. (2) {\em Data-driven Cooperative Task Allocation (DCTA) Module} captures the dynamic task importance and allocates tasks with data-driven techniques, which has been introduced in detail in Section \ref{Sec:Model}. (3) {\em Traditional Prediction Module} executes the data-driven prediction tasks at the edge nodes and outputs the prediction results. (4) {\em Decision Making Module} receives the prediction results from the multiple edge nodes and conducts the optimal decision which is to maximize the overall system merit.}

{The DCTA modules for task allocation lies in the Controller and the design is introduced in previous Section \ref{Sec:Model}. In the following, we are to briefly introduce the design of other components, i.e., {\em data collecting module}, {\em traditional prediction module}, and {\em decision making module}, within our chiller AIOps system architecture.}


{\textbf{Data Collecting Module.} The module lies in the Sensing Nodes, e,.g, the temperature sensor or humidity sensor, which collects the data from the surroundings for analysis. There exist a common data storage problem due to the storage limitations on these edge nodes. To tackle this problem, we keep uploading data to a more powerful edge node, e.g., gateway or server, and overwrite historical data on these edge nodes when the storage is insufficient.}

{\textbf{Traditional Prediction Module.} The module lies in the Operation Nodes, e.g., gateway or router, which executes data-driven COP prediction tasks and outputs the prediction results. To ensure the accuracy of each data-driven task in the case of data scarcity on these edge nodes, we apply clustered multi-task learning approach \cite{jacob09}. It learns with training data not only from the target task, but also from other tasks, e.g., cases with similar temporal, meteorological and mechanical conditions.}


{\textbf{Decision Making Module.} The module lies in the Controller or Operation Nodes, e.g., server or gateway, which should work in an iterative optimization way. Under the circumstance, the frequency of the decision update is then critical to edge nodes network resource utilization and energy consumption. To tackle this problem, we propose an efficient algorithm to determine the frequency of decision update by analyzing the historical decision data. Specifically, we update the decision each time when an industrial demand coming. In order to reduce damage to the system, we ensure that the time interval between the two decisions can meet the needs of the system to transition from one steady state to another. As for the effects of varying this frequency, it would be an interesting future work for us to investigate the optimal frequency of decision update in industrial scenarios.}




\subsection{Experiment Results}

\textbf{Result on Overall Merit.}
{With the chiller AIOps system, we first compare the overall merit of our data-driven cooperative task allocation (DCTA) with that of the other state-of-the-art task allocation methods. Figure~\ref{fig:merit} shows that, on one hand, our DCTA approach and other state-of-the-art methods can eventually achieve the same performance; on the other hand, with the same performance, our DCTA approach can greatly reduce the number of tasks performed which means significant savings in time and resources. That is because our DCTA approach is developed combined with the runtime data in the real environment and a huge amount of simulation data. In addition, it leverages the ensemble technique to avoid overfitting in non-linear modeling, which can successfully capture the system local and dynamic performance.}

\textbf{Result on Processing Time.}
{To show the potential of saving time, We compare the processing time of the state-of-the-art task allocation methods. In Fig. \ref{fig:time}, we can see that our DCTA outperforms RM, DML, and CRL by 50.2\%, 38.6\% and 30.2\%, respectively. That is because DCTA uses data-driven allocation to select the most important tasks for prediction, unlike other non-data-driven methods.}


\textbf{Result on Energy Consumption.}
{Figure \ref{fig:energy} compares our DCTA approach with RM, DML and CRL method over a different number of tasks, in terms of Average Energy Consumption on edge devices. On average, our DCTA outperforms RM, DML and CRL by 48.4\%, 39.6\% and 31.3\%, respectively. That is because not all predictions on all operations are necessary. Our DCTA captures the top important operations and still maintains the superiority of data-driven techniques.}









% \begin{figure*}[t]
% 	\begin{minipage}[htpb]{0.32\linewidth}
% 		\centering
% 		%\vspace{-0.1cm}
% 		\includegraphics[width=2.2in]{new-figure/topology.pdf}
% 		\vspace{-0.2cm}
% 		\caption{The network topology of Chiller AIOps System on the Edge. \label{fig:topology}}
% 	\end{minipage}
% 	\hfill
% 	\begin{minipage}[htpb]{0.32\linewidth}
% 		\centering
% 		%\vspace{-0.2cm}
% 		\includegraphics[width=2.3in]{new-figure/hardware.pdf}
% 		\vspace{-0.7cm}
% 		\caption{The hardware choices of C-node, O-node and S-node, respectively. \label{fig:hardware}}
% 	\end{minipage}
% 	\hfill
% 	\begin{minipage}[htpb]{0.32\linewidth}
% 		\centering
% 		%\vspace{-0.2cm}
% 		\includegraphics[width=2.5in]{new-figure/framework-new.pdf}
% 		\vspace{-0.5cm}
% 		\caption{Framework of Chiller AIOps System on the Edge. \label{fig:framework}}
% 	\end{minipage}
% 	\hfill
% \vspace{-0.3cm}
% \end{figure*}

% \subsection{Hardware Choices}
% To apply our DCTA approach to the chiller AIOps system, we briefly introduce the hardware choices corresponding to the network topology of Fig. 12 on the edge.

% \textbf{The C-Node:} We use a laptop with 6 cores of 2.8 GHz CPU, and a total memory of 8 GB as the controller (Fig. \ref{fig:hardware}). 

% \textbf{The O-Node:} We use Raspberry Pi 3 Model A+, Raspberry Pi 3 Model B and Raspberry Pi 3 Model B+ as the O-node hardware board (Fig. \ref{fig:hardware}) by considering the different processing capacity of hardware board on different edge devices. For example, for Model A+ equipped with 4 BCM2837B0 cores of 1.4 GHz CPU and 512 MB memory, while Model B equipped with 4 BCM2837 cores of 1.2 GHz CPU and 1 GB memory. They are have linux operating systems that match this hardware feature and we use IEEE 802.11.b/g/n/ac Wireless LAN for communication. 

% \textbf{The S-Node:} We use a Raspberry Pi 3 Model A+ as the S-node platform (Fig. \ref{fig:hardware}). Due to the lack of a variety of sensors on hand, we store the data collected by the major building provider and simulate the data collection process. We also use IEEE 802.11.b/g/n/ac Wireless LAN for communication.



%In this section, we first introduce the formal definition of our problem and then the corresponding solution framework. 

% % {Updated: 1. the section of Framework; 2. Structure; 3. $x_i$ and $x_{ijr}$; 4. i = 1 ,..., N; 5. define variable explicitly; 6. task definition; 7. where and which; 8. remove implementation details in problem, e.g., RL methods or chillers.}

% % \todo{1. Why r is also 1 - N, which is the same as i? Do we assume that one task can be run on only one processor, instead of two or half processor? If so, why is it reasonable? 2. what is given in our problem? 3. Empty space in boxes of the framework figure.}

% \subsection{Problem Formulation}


% % \todo{We may merely formulate the data-driven task ordering problem, leaving the other components in the case study section.}

% \subsubsection{Basic Notations}
% Before introducing our problem, we first define the basic concepts and the notation system. 


% \textbf{Local Processor and Edge Server.} We consider a generic edge computing system consisting of a finite number of heterogeneous local processors and an edge server. The local processors can present the processing cores in a single user equipment (e.g. sensors). These processors may have different speeds but are assumed to be unary, i.e., each processor executes one task at a time, while the other tasks assigned to the processor wait in a queue. %{We emphasize that, with respect to the cost and delay in task processing, this assumption is without loss of generality.\footnote{It is easy to see that there is no benefit in processor-sharing with respect to sum queueing-and-execution delay of the tasks.}} \todo{It is not clear that there will be no benefit for sharing: at least the computation of top tasks can be accelerated. Please rewrite the justification.}
 
% We further assume the edge server that also provides an essentially finite number of processors, which can be viewed as an additional processor that can process up to $K'$ tasks simultaneously. Let the set of all processors, including the edge server, be $\mathbb{P}$ and its size be $M$. Additionally, let $s_j$ represents the processing speed of processor $j$, where $j \in \{1, ..., M\}$ denotes the index of processors. 

% \textbf{Task Definition.} Consider a single data-driven application that must be completed before a deadline $T_D$. The application is partitioned into multiple machine learning \emph{tasks}, whose dependency is sharing the similar training samples. A \emph{task} is defined as a set of data and the corresponding prediction model for a specific context. For example, in the industrial sector, a set of configurations and the corresponding prediction model of industrial performance is a task. 

% Let $N$ denote the total number of tasks and $d_i$ represents the input-data size of task $i$, where $i \in \{1, ..., N\}$ denotes the index of tasks. Then, we assume that an application is initialed at a particular local processor and must end at the same local processor. In other words, there is an initial task (task $1$) that starts the application and a final task (task $N$) that terminates it.

% If task $i$ is executed on processor $j$, the execution time is $t_{ij}$ which is correspond to $d_i/s_j$. In this work, we proceed assuming that such information is already given.\footnote{In practice, the processing times and data transfer requirement may be obtained by applying a program profile as shown in experimental studies such as MAUI \cite{cuervo2010maui} and Thinkair \cite{kosta2012thinkair}.}


% \subsubsection{Formal Definition.} With the above notations, we formally define our problem, including the decision variables, models and related constraints.

% \textbf{Decision Variable and Constraints.} Our task scheduling decision is to achieve both the mapping between tasks and processors and the order of the tasks execution in each processor. 

% First, we define the scheduling decision variables as follows:\\

% $x_{ijr} := 
% \begin{cases} 
% 1, & \mbox{if task } i \mbox{ is on processor } j \mbox{ in position } r 
% \\ 0, & \mbox{if otherwise}
% \end{cases} \\
% $    \\ 
% Meantime, the output of model $x_{ijr} \in \{0,1\}$ denotes task $i$ is assigned to processor $j$ in position $r$, where $r \in \{1, ..., K\}$ denotes the index of position. Each task is to be scheduled to exactly one of the existing positions on the processors. Hence,

% \begin{eqnarray}
% \sum_{j=1}^M \sum_{r=1}^K x_{ijr} = 1,\ \ \ \ \forall \mbox{$i \in \{1, \ldots, N$} \}. 
% \end{eqnarray}


% Furthermore, each position on each processor can be assigned to at most one task, which is given by 

% \begin{eqnarray}
% \sum_{i=1}^N x_{ijr} \leq 1,\ \ \ \ \forall \mbox{$r \in \{1,\ldots,K\}$, $j \in \{1,\ldots, M\}$.} 
% \end{eqnarray}

% \textbf{Models and Constraints.} In our scenario, the result of each task has different importance to the decision-making of achieving the industrial goal. As mention in the motivation section, our observation exposing that not all prediction tasks are valuable to execute in terms of the limited computation time and resources. Facing the above situation, we propose a {\em data-driven model} $\mathcal{F(\cdot)}$ to obtain the priority of each task. Hence,

% \begin{eqnarray}
% \mathcal{F(\mbox{$i$,$w_i$})} = p_i,\ \ \ \ \forall \mbox{$i \in \{1, \ldots,N\}$,}  
% \end{eqnarray}
% where $w_i$ denotes the features of the corresponding task $i$; the output $p_i$ of the above model denotes the priority of task $i$. 

==> DCTA-model.tex <==
\section{CRL-based Local Process with a Cooperative Learning Framework} 
In this section, we first show that the CRL model should not be directly applied due to the simulation limitations. We then propose a Cooperative Learning approach based on both CRL and Support Vector Machine (SVM) to fully leverage the simulated and real-world data. At last, we briefly introduce the design of the SVM model. 

\subsection{Introducing Local Process with Cooperative Learning}
In the previous section, we present a detailed design of the CRL model. However, the CRL model should not be directly applied. In our scenario, the environment is diverse over time. Although we can find similar environments in the historical environment through simple clustering methods, there is a risk that the environment is still not closed to the real environment. That is especially true for edge devices without too much data, whereas the RL model can confront with quite a few unseen environments and it requires much environment observations to cover all possible situations.  


In this regard, directly leveraging the CRL model can still mismatch the environment and submitted less important tasks, which leads to poor decision performance \cite{hu2018synthesize}. We also conduct an experiment to demonstrate the negative impact. Based on our CRL model, when the environment is not accurate, it leads to a 28.84\% reduction of performance. 


 
To tackle the challenge, our idea is to leverage runtime data to adjust the decision of the CRL model.



Accordingly, we propose a cooperative learning approach as shown in Fig. \ref{fig:Clearning}, which is especially well-suited to solve this problem. The proposed cooperative learning approach contains two components: 1) a general process with a huge environment definition data, and 2) a local process with few real-world data. Formally, let $\mathcal{C}$ and $\mathcal{R}$ be the feature spaces of the environment definition data, i.e., $\mathcal{C} = \{(e,s_0)\}$, and real-world data, respectively. Let $\mathcal{F}(\cdot)$ denotes our cooperative learning model, which can be represented more specifically as: 
\begin{eqnarray}
\mathcal{F}(\textbf{J},\mathcal{X}) = \mathcal{F}(\textbf{J},(\mathcal{C},\mathcal{R})) = w_1\mathcal{F}_1{(\textbf{J}, \mathcal{C})}   + w_2\mathcal{F}_2{(\textbf{J}, \mathcal{R})},  
\end{eqnarray}
where $\mathcal{F}_1(\cdot)$ and $\mathcal{F}_2(\cdot)$ denote the general process and local process; $w_1$ and $w_2$ denote the weight of the corresponding model results, respectively. In addition, the task-allocation matrix $\textbf{u}$ is outputted by our cooperative learning model $\mathcal{F}(\cdot)$, i.e., $\textbf{u} \leftarrow \mathcal{F}(\textbf{J},(\mathcal{C},\mathcal{R}))$.

\subsection{Brief Design of Local Process}
For our cooperative learning, We have discussed the first component of the general process using CRL in the previous section. Now we introduce the design of the local process.

As for the second component of local process, we compare several state-of-the-art models of SVM, AdaBoost, and Random Forest. We select SVM because of its highest accuracy. Formally, given the target tasks feature values $\mathcal{X}$, our objective is to develop an SVM predictor $\mathcal{F}_2(\cdot)$ which infers the target tasks allocation $\textbf{u}$. This can be formulated as follows:
\begin{eqnarray}
\textbf{u} \leftarrow  \mathcal{F}_2(\textbf{J},\mathcal{X}) = \emph{SVM}(\mathcal{X};w,\textbf{J})
\end{eqnarray}
where $w$ denotes its parameter vector. 
%\revised{For the interested reader, the design of loss function and feature engineering can be found in Appendix B of our technique report \cite{Technical-report}.}


In the following, we are to briefly introduce the design of loss function and feature engineering of the local process of SVM predictor.

\begin{figure}[t]
\centering
\vspace{-0.1cm}
\includegraphics[angle=0, width=0.43\textwidth]{figures/c-learning.pdf}
\vspace{-0.1cm}
\caption{Framework of Cooperative Learning for task allocation.}
\label{fig:Clearning}
\vspace{-0.5cm}
\end{figure}


\subsection{Loss Function of Local Process}
Formally, let $\mathcal{R}$ be the feature spaces of the real-world data, sample $k \in \mathcal{R}$ usually consists of two parts. One is a vector $x_k$ that is regarded as the input feature values; the other is a scalar $y_k$ that is the desired output of the model. Then, we define the loss function $\mathcal{L}_k(w)$ of our SVM predictor $\mathcal{F}_2(\cdot)$ as follows:
\begin{eqnarray}
\mathcal{L}_k(w) =  \frac{1}{2}\Vert w \Vert ^2 + \frac{1}{2} \textrm{max} \{0; 1 - y_k w^T x_k \} ^2,
\end{eqnarray}
where $w$ denotes its parameter vector; $w^T$ denotes the transpose of $w$ and $\Vert \cdot \Vert ^2$ denotes the $\mathcal{L}^2$ norm.
Finally, our optimization process is to find the optimal parameter vector $w^*$ that minimize the loss function $\mathcal{L}_k(w)$ on a collection of training dataset $\mathcal{R}$. Hence, $w^* = \arg \min \frac{1}{\vert \mathcal{R} \vert}\sum_{k \in \mathcal{R}} \mathcal{L}_k(w)$.


\begin{table*}[ht]\footnotesize \centering
\vspace{-0.1cm}
\caption{The description of features in the local process of SVM predictor.}
\label{table:features} 
\vspace{-0.1cm}
\begin{tabular}{|c|c|c|}
\hline
Feature Type & Feature & Description  \\
\hline
\hline
\multirow{2}{*}{General} & Past Success & The number of cases that a task is selected in the optimal decision in the past \\
\cline{2-3}
& Prediction Accuracy & The similarity between the predicted (e.g., COP) and the real for a task in the past \\
\hline
\multirow{8}{*}{Domain}
& Building & The building that the operating chiller is deployed in  \\
\cline{2-3}
& Model Type & The model of the operating chiller  \\
\cline{2-3}
& Operating Power & The power measured by kilowatts for the operating chiller  \\
\cline{2-3}
& Weather Condition & The description of weather condition in a time interval  \\
\cline{2-3}
& Outdoor Temperature & The outdoor temperature measured by Celsius in a time interval \\
\cline{2-3}
& Latest Cooling Load & The last recorded cooling load assigned on this chiller \\
\cline{2-3}
& Water Mass Flow Rate & The mass of water flowing per second, measured by kg/s \\
\cline{2-3}
 & Water Temperature Difference & The difference between the returned and supplied chilled water temperature \\
\hline
\end{tabular}
\vspace{-0.4cm}
\end{table*}

\subsection{Feature Engineering of Local Process}
In most real-world scenarios, e.g., industry domain, it is either costly or even impossible to obtain the data on environments and configurations of tasks; we usually do not have the luxury to obtain enormous data where local predictor can be trained with irrelevant features automatically eliminated. As such the challenge is to select the proper feature set for our local predictor. Thus, we propose a domain-assisted feature engineering approach which uses domain knowledge to create features relevant to the problem at hand. The feature set consists of the following two types of features, naming domain features and general features, respectively. We list our features in Table \ref{table:features}.


\textbf{General features.} Overall, the general features should have some universality and can be easily applied to other scenarios. More specifically, it should reflect the decision performance of a data-driven task in the statistical view over the historical data. We consider the following two factors: 1) Past Success which refers to the number of cases that a task is selected in the optimal decision in the past. In general, if the industrial demand, configuration, and environment do not change too much, a task selected in the past will likely be selected again in the current period; 2) Prediction Accuracy which is the similarity between the predicted performance and the real performance for a given task in the past. This is also an important factor since an accurate prediction indicates our final decision making can be more reliable.

\textbf{Domain features.} Obviously, the domain features are closely related to specific scenarios. Recall the previous example in the driver-less car, driving operation decision is critical to driver-less car safety, which consists of the following specific characteristics such as engine status, speed, radar data, GPS data and etc. While in this paper, we focus on the industrial field where chiller sequencing is a common but highly important industrial operation in energy-efficient buildings, which consists of the following specific features: 1) Meteorological information such as temperature and weather drive the cooling demand imposed on the chillers; 2) Mechanical information such as the model type, building, operating power, water temperature difference, flow rate, and the recent cooling load are used to capture the chiller specific characteristics.



%\todo{Add a table of all used features and their description.}\revised{revised}

%\todo{Further introduce general features, e.g., what are past success, prediction accuracy and etc, and why do we use them.}\revised{revised}

